A review of approaches to modeling applied vehicle routing problems

Due to the practical importance of vehicle routing problems (VRP), there exists an ever-growing body of research in algorithms and (meta)heuristics for solving such problems. However, the diversity of VRP domains creates the separate problem of modeling such problems -- describing the domain entities (and, in particular, the planning decisions), the set of valid planning decisions, and the preferences between different plans. In this paper, we review the approaches for modeling vehicle routing problems. To make the comparison more straightforward, we formulate several criteria for evaluating modeling methods reflecting the practical requirements of the development of optimization algorithms for such problems. Finally, as a result of this comparison, we discuss several future research avenues in the field of modeling VRP domains.

==> mind-map.tex <==

\begin{tikzpicture}[
  mindmap, grow cyclic,
  every node/.style=concept,
  every node/.append style={execute at begin node=\hskip0pt},
  concept color=orange!40,
	level 1/.append style={
	  sibling angle=90,
	  font=\normalsize,
    minimum size=2.5cm,
    text width=2.25cm,
	  level distance=4cm,
  },
	level 2/.append style={
	  sibling angle=75,
	  font=\normalsize,
    minimum size=2.35cm,
    text width=2.1cm,
    level distance=3.5cm,
	},
	level 3/.append style={
	  sibling angle=70,
    font=\small,
    minimum size=2.25cm,
    text width=2cm,
    level distance=3.25cm
	},
	level 4/.append style={
	  sibling angle=45,
    font=\small,
    minimum size=2.25cm,
    text width=2cm,
    level distance=3.25cm
	},
]

\node[minimum size=2.5cm,text width=2.25cm]{VRP algorithms}
child [concept color=blue!30, level distance=3.4cm] { node {Mathematical programming}
	child { node {Constraint programming}}
	child { node {Mixed-integer programming}
	  child { node [align=center] {Flow \\ formulations}}
	  child { node [align=center] {Set \\ partitioning formulations}}
	}
}
child [concept color=purple!50] { node {Heuristic algorithms}
	child [concept color=purple!40] { node {Constructive heuristics}
	  child [
	    concept color=purple!25,
      sibling angle=40,
      minimum size=1.5cm,
      text width=1.5cm,
    ] { node {\dots} }
	  child { node {Nearest neighbor}}
	  child { node {Savings algorithm}}
	}
	child [concept color=purple!60] { node {Metaheuristics}
	  child [
	    concept color=purple!25,
      sibling angle=40,
      minimum size=1.5cm,
      text width=1.5cm,
    ] { node {\dots} }
	  child { node {Local search}
	    child { node {Large neighborhood search}}
	    child { node {Simulated annealing}}
	    child { node {Tabu search}}
	  }
	  child { node {Evolutionary algorithms}
	    child { node {Genetic algorithms}}
	    child { node {Ant colony optimization}}
	    child { node {Particle swarm optimization}}
	  }
	}
}
child [concept color=teal!40, level distance=3.4cm] { node {Machine learning approaches}
	child { node {End to end learning}}
	child { node {Learning to configure}}
	child { node [align=center] {ML \\ alongside \\ algorithms}}
};

\end{tikzpicture}


